Afterglow Observations of Fermi-LAT Gamma-Ray Bursts and the Emerging Class of Hyper-Energetic Events

We present broadband (radio, optical, and X-ray) light curves and spectra of the afterglows of four long-duration gamma-ray bursts (GRBs 090323, 090328, 090902B, and 090926A) detected by the Gamma-Ray Burst Monitor (GBM) and Large Area Telescope (LAT) instruments on the Fermi satellite. With its wide spectral bandpass, extending to GeV energies, Fermi is sensitive to GRBs with very large isotropic energy releases (10e54 erg). Although rare, these events are particularly important for testing GRB central-engine models. When combined with spectroscopic redshifts, our afterglow data for these four events are able to constrain jet collimation angles, the density structure of the circumburst medium, and both the true radiated energy release and the kinetic energy of the outflows. In agreement with our earlier work, we find that the relativistic energy budget of at least one of these events (GRB 090926A) exceeds the canonical value of 10e51 erg by an order of magnitude. Such energies pose a severe challenge for models in which the GRB is powered by a magnetar or neutrino-driven collapsar, but remain compatible with theoretical expectations for magneto-hydrodynamical (MHD) collapsar models. Our jet opening angles (theta) are similar to those found for pre-Fermi GRBs, but the large initial Lorentz factors (Gamma_0) inferred from the detection of GeV photons imply theta Gamma_0 ~ 70-90, values which are above those predicted in MHD models of jet acceleration. Finally, we find that these Fermi-LAT events preferentially occur in a low-density circumburst environment, and we speculate that this might result from the lower mass-loss rates of their lower-metallicity progenitor stars. Future studies of Fermi-LAT afterglows in the radio with the order-of-magnitude improvement in sensitivity offered by the EVLA should definitively establish the relativistic energy budgets of these events.

==> tab1.tex <==
\ProvidesFile{0926aopt.tab.tex}

\LongTables
\begin{deluxetable}{lccccc}
\tabletypesize{\scriptsize}
\tablecaption{Optical/NIR observations of \grbd}
\tablewidth{0pt}
\tablehead{
\colhead{Date\tablenotemark{a}} & \colhead{Time Since Burst\tablenotemark{b}} & \colhead{Telescope/Instrument} & \colhead{Filter} &  \colhead{Exposure Time} & \colhead{Magnitude\tablenotemark{c}} \\
\colhead{(UT)} & \colhead{(d)} & & \colhead{(s)} &
}
\startdata
%
2009 Sep 26.72 & 0.5415 & UVOT & $U$ & 358.0 & $18.33 \pm 0.06$ \\
2009 Sep 26.72 & 0.5501 & UVOT & $V$ & 358.0 & $18.34 \pm 0.10$ \\
2009 Sep 26.78 & 0.5989 & UVOT & $U$ & 675.0 & $18.50 \pm 0.05$ \\
2009 Sep 26.79 & 0.6149 & UVOT & $V$ & 675.0 & $18.91 \pm 0.09$ \\
2009 Sep 26.84 & 0.6649 & UVOT & $U$ & 704.5 & $18.71 \pm 0.05$ \\
2009 Sep 26.85 & 0.6816 & UVOT & $V$ & 703.3 & $19.09 \pm 0.10$ \\
2009 Sep 26.90 & 0.7299 & UVOT & $U$ & 526.0 & $18.84 \pm 0.07$ \\
2009 Sep 26.96 & 0.7966 & PROMPT-2 & $V$ & 560.0 & $18.76 \pm 0.22$ \\
2009 Sep 26.96 & 0.7969 & PROMPT-4 & $R$ & 640.0 & $18.69 \pm 0.16$ \\
2009 Sep 26.96 & 0.7986 & PROMPT-5 & $I$ & 400.0 & $18.02 \pm 0.19$ \\
2009 Sep 26.98 & 0.8062 & UVOT & $U$ & 459.4 & $18.94 \pm 0.08$ \\
2009 Sep 26.99 & 0.8172 & UVOT & $V$ & 459.4 & $18.97 \pm 0.12$ \\
2009 Sep 27.00 & 0.8250 & PROMPT-5 & $I$ & 720.0 & $18.12 \pm 0.07$ \\
2009 Sep 27.00 & 0.8259 & PROMPT-4 & $R$ & 880.0 & $18.49 \pm 0.05$ \\
2009 Sep 27.00 & 0.8314 & PROMPT-2 & $V$ & 1600.0 & $19.12 \pm 0.10$ \\
2009 Sep 27.00 & 0.8372 & PROMPT-5 & $I$ & 880.0 & $18.06 \pm 0.05$ \\
2009 Sep 27.00 & 0.8379 & PROMPT-4 & $R$ & 880.0 & $18.45 \pm 0.04$ \\
2009 Sep 27.00 & 0.8553 & PROMPT-4 & $R$ & 800.0 & $18.41 \pm 0.04$ \\
2009 Sep 27.00 & 0.8553 & PROMPT-5 & $I$ & 800.0 & $18.04 \pm 0.05$ \\
2009 Sep 27.00 & 0.8583 & SMARTS / ANDICAM & $I$ & 2160.0 & $18.17 \pm 0.07$ \\
2009 Sep 27.00 & 0.8583 & SMARTS / ANDICAM & $J$ & 1800.0 & $17.28 \pm 0.07$ \\
2009 Sep 27.00 & 0.8603 & PROMPT-2 & $V$ & 1520.0 & $19.12 \pm 0.09$ \\
2009 Sep 27.04 & 0.8654 & PROMPT-3 & $B$ & 880.0 & $19.56 \pm 0.10$ \\
2009 Sep 27.04 & 0.8659 & PROMPT-4 & $R$ & 800.0 & $18.36 \pm 0.04$ \\
2009 Sep 27.04 & 0.8660 & PROMPT-5 & $I$ & 800.0 & $17.97 \pm 0.05$ \\
2009 Sep 27.04 & 0.8662 & UVOT & $U$ & 689.8 & $18.80 \pm 0.06$ \\
2009 Sep 27.04 & 0.8761 & PROMPT-4 & $R$ & 800.0 & $18.36 \pm 0.04$ \\
2009 Sep 27.04 & 0.8764 & PROMPT-5 & $I$ & 640.0 & $17.95 \pm 0.05$ \\
2009 Sep 27.04 & 0.8808 & PROMPT-2 & $V$ & 1520.0 & $19.19 \pm 0.09$ \\
2009 Sep 27.04 & 0.8811 & PROMPT-3 & $B$ & 1520.0 & $19.57 \pm 0.07$ \\
2009 Sep 27.05 & 0.8826 & UVOT & $V$ & 689.7 & $18.86 \pm 0.09$ \\
2009 Sep 27.04 & 0.8858 & PROMPT-5 & $I$ & 800.0 & $17.87 \pm 0.04$ \\
2009 Sep 27.04 & 0.8864 & PROMPT-4 & $R$ & 800.0 & $18.31 \pm 0.04$ \\
2009 Sep 27.04 & 0.8962 & PROMPT-5 & $I$ & 800.0 & $17.92 \pm 0.05$ \\
2009 Sep 27.04 & 0.8967 & PROMPT-4 & $R$ & 800.0 & $18.29 \pm 0.04$ \\
2009 Sep 27.04 & 0.9012 & PROMPT-3 & $B$ & 1600.0 & $19.56 \pm 0.07$ \\
2009 Sep 27.04 & 0.9013 & PROMPT-2 & $V$ & 1520.0 & $19.02 \pm 0.08$ \\
2009 Sep 27.08 & 0.9055 & PROMPT-5 & $I$ & 640.0 & $17.85 \pm 0.05$ \\
2009 Sep 27.08 & 0.9065 & PROMPT-4 & $R$ & 720.0 & $18.34 \pm 0.04$ \\
2009 Sep 27.08 & 0.9172 & PROMPT-4 & $R$ & 880.0 & $18.29 \pm 0.04$ \\
2009 Sep 27.08 & 0.9172 & PROMPT-5 & $I$ & 880.0 & $17.72 \pm 0.03$ \\
2009 Sep 27.08 & 0.9223 & PROMPT-3 & $B$ & 1680.0 & $19.38 \pm 0.05$ \\
2009 Sep 27.08 & 0.9225 & PROMPT-2 & $V$ & 1600.0 & $18.95 \pm 0.07$ \\
2009 Sep 27.08 & 0.9280 & PROMPT-4 & $R$ & 800.0 & $18.29 \pm 0.04$ \\
2009 Sep 27.08 & 0.9284 & PROMPT-5 & $I$ & 560.0 & $17.85 \pm 0.05$ \\
2009 Sep 27.10 & 0.9331 & UVOT & $U$ & 691.7 & $18.64 \pm 0.05$ \\
2009 Sep 27.08 & 0.9388 & PROMPT-4 & $R$ & 880.0 & $18.15 \pm 0.03$ \\
2009 Sep 27.08 & 0.9388 & PROMPT-5 & $I$ & 880.0 & $17.76 \pm 0.04$ \\
2009 Sep 27.08 & 0.9419 & PROMPT-3 & $B$ & 1360.0 & $19.56 \pm 0.08$ \\
2009 Sep 27.08 & 0.9421 & PROMPT-2 & $V$ & 1280.0 & $18.85 \pm 0.08$ \\
2009 Sep 27.13 & 0.9475 & PROMPT-4 & $R$ & 480.0 & $18.25 \pm 0.05$ \\
2009 Sep 27.13 & 0.9477 & PROMPT-5 & $I$ & 480.0 & $17.82 \pm 0.05$ \\
2009 Sep 27.12 & 0.9495 & UVOT & $V$ & 691.7 & $18.76 \pm 0.09$ \\
2009 Sep 27.17 & 0.9933 & PROMPT-3 & $B$ & 960.0 & $19.60 \pm 0.07$ \\
2009 Sep 27.17 & 0.9933 & PROMPT-5 & $I$ & 960.0 & $17.82 \pm 0.04$ \\
2009 Sep 27.17 & 0.9935 & PROMPT-2 & $V$ & 960.0 & $18.88 \pm 0.10$ \\
2009 Sep 27.17 & 0.9938 & PROMPT-4 & $R$ & 1040.0 & $18.21 \pm 0.03$ \\
2009 Sep 27.17 & 0.9992 & UVOT & $U$ & 554.0 & $18.65 \pm 0.06$ \\
2009 Sep 27.17 & 1.0058 & PROMPT-5 & $I$ & 960.0 & $17.83 \pm 0.03$ \\
2009 Sep 27.17 & 1.0062 & PROMPT-4 & $R$ & 880.0 & $18.24 \pm 0.03$ \\
2009 Sep 27.17 & 1.0100 & PROMPT-3 & $B$ & 1200.0 & $19.43 \pm 0.06$ \\
2009 Sep 27.17 & 1.0107 & PROMPT-2 & $V$ & 1520.0 & $19.03 \pm 0.09$ \\
2009 Sep 27.17 & 1.0166 & PROMPT-4 & $R$ & 560.0 & $18.19 \pm 0.04$ \\
2009 Sep 27.17 & 1.0173 & PROMPT-5 & $I$ & 640.0 & $17.79 \pm 0.04$ \\
2009 Sep 27.21 & 1.0293 & PROMPT-4 & $R$ & 960.0 & $18.26 \pm 0.03$ \\
2009 Sep 27.21 & 1.0295 & PROMPT-5 & $I$ & 880.0 & $17.85 \pm 0.04$ \\
2009 Sep 27.21 & 1.0352 & PROMPT-2 & $V$ & 1680.0 & $18.89 \pm 0.07$ \\
2009 Sep 27.21 & 1.0363 & PROMPT-3 & $B$ & 1360.0 & $19.53 \pm 0.07$ \\
2009 Sep 27.21 & 1.0408 & PROMPT-5 & $I$ & 800.0 & $17.87 \pm 0.04$ \\
2009 Sep 27.21 & 1.0412 & PROMPT-4 & $R$ & 880.0 & $18.43 \pm 0.04$ \\
2009 Sep 27.21 & 1.0530 & PROMPT-5 & $I$ & 960.0 & $18.01 \pm 0.04$ \\
2009 Sep 27.21 & 1.0530 & PROMPT-4 & $R$ & 960.0 & $18.42 \pm 0.04$ \\
2009 Sep 27.21 & 1.0590 & PROMPT-2 & $V$ & 1840.0 & $19.13 \pm 0.10$ \\
2009 Sep 27.21 & 1.0592 & PROMPT-3 & $B$ & 1920.0 & $19.64 \pm 0.06$ \\
2009 Sep 27.21 & 1.0653 & PROMPT-4 & $R$ & 960.0 & $18.43 \pm 0.04$ \\
2009 Sep 27.21 & 1.0655 & PROMPT-5 & $I$ & 960.0 & $18.00 \pm 0.05$ \\
2009 Sep 27.24 & 1.0658 & UVOT & $U$ & 730.1 & $18.67 \pm 0.05$ \\
2009 Sep 27.25 & 1.0777 & PROMPT-4 & $R$ & 960.0 & $18.56 \pm 0.04$   \\
2009 Sep 27.25 & 1.0780 & PROMPT-5 & $I$ & 960.0 & $18.02 \pm 0.04$   \\
2009 Sep 27.25 & 1.0839 & PROMPT-3 & $B$ & 1920.0 & $19.59 \pm 0.05$   \\
2009 Sep 27.25 & 1.0839 & PROMPT-2 & $V$ & 1840.0 & $19.15 \pm 0.09$   \\
2009 Sep 27.25 & 1.0900 & PROMPT-4 & $R$ & 960.0 & $18.45 \pm 0.03$   \\
2009 Sep 27.25 & 1.0902 & PROMPT-5 & $I$ & 880.0 & $17.97 \pm 0.04$   \\
2009 Sep 27.25 & 1.1028 & PROMPT-5 & $I$ & 1040.0  & $17.98 \pm 0.04$   \\
2009 Sep 27.25 & 1.1029 & PROMPT-4 & $R$ & 1040.0 & $18.39 \pm 0.03$   \\
2009 Sep 27.25 & 1.1091 & PROMPT-3 & $B$ & 2000.0 & $19.51 \pm 0.04$   \\
2009 Sep 27.25 & 1.1093 & PROMPT-2 & $V$ & 1920.0 & $18.96 \pm 0.07$   \\
2009 Sep 27.29 & 1.1158 & PROMPT-4 & $R$ & 960.0 & $18.47 \pm 0.03$   \\
2009 Sep 27.29 & 1.1158 & PROMPT-5 & $I$ & 960.0 & $18.04 \pm 0.04$   \\
2009 Sep 27.29 & 1.1283 & PROMPT-5 & $I$ & 960.0 & $18.02 \pm 0.04$   \\
2009 Sep 27.29 & 1.1287 & PROMPT-4 & $R$ & 1040.0 & $18.45 \pm 0.03$   \\
2009 Sep 27.29 & 1.1348 & PROMPT-3 & $B$ & 2000.0 & $19.62 \pm 0.05$   \\
2009 Sep 27.29 & 1.1352 & PROMPT-2 & $V$ & 1920.0 & $19.09 \pm 0.09$   \\
2009 Sep 27.29 & 1.1413 & PROMPT-5 & $I$ & 1040.0 & $17.97 \pm 0.04$   \\
2009 Sep 27.29 & 1.1415 & PROMPT-4 & $R$ & 960.0 & $18.43 \pm 0.03$   \\
2009 Sep 27.33 & 1.1545 & PROMPT-4 & $R$ & 960.0 & $18.47 \pm 0.03$   \\
2009 Sep 27.33 & 1.1550 & PROMPT-5 & $I$ & 1040.0 & $18.06 \pm 0.05$   \\
2009 Sep 27.33 & 1.1617 & PROMPT-2 & $V$ & 2000.0 & $19.11 \pm 0.07$   \\
2009 Sep 27.33 & 1.1617 & PROMPT-3 & $B$ & 2080.0 & $19.67 \pm 0.06$   \\
2009 Sep 27.33 & 1.1684 & PROMPT-4 & $R$ & 1040.0 & $18.51 \pm 0.03$ \\
2009 Sep 27.33 & 1.1685 & PROMPT-5 & $I$ & 1040.0 & $18.06 \pm 0.05$ \\
2009 Sep 27.33 & 1.1818 & PROMPT-4 & $R$ & 1040.0 & $18.52 \pm 0.04$ \\
2009 Sep 27.33 & 1.1826 & PROMPT-5 & $I$ & 960.0 & $18.24 \pm 0.06$ \\
2009 Sep 27.33 & 1.1850 & PROMPT-3 & $B$ & 1520.0 & $19.74 \pm 0.08$ \\
2009 Sep 27.33 & 1.1859 & PROMPT-2 & $V$ & 1600.0 & $19.05 \pm 0.10$ \\
2009 Sep 27.33 & 1.1919 & PROMPT-4 & $R$ & 480.0 & $18.63 \pm 0.07$ \\
2009 Sep 27.33 & 1.1923 & PROMPT-5 & $I$ & 480.0 & $18.28 \pm 0.11$ \\
2009 Sep 27.38 & 1.2093 & PROMPT-3 & $B$ & 480.0 & $19.73 \pm 0.19$ \\
2009 Sep 27.38 & 1.2093 & PROMPT-4 & $R$ & 480.0 & $18.71 \pm 0.08$ \\
2009 Sep 27.38 & 1.2093 & PROMPT-5 & $I$ & 480.0 & $18.18 \pm 0.10$ \\
2009 Sep 27.38 & 1.2095 & PROMPT-2 & $V$ & 480.0 & $18.97 \pm 0.23$ \\
2009 Sep 27.84 & 1.6702 & UVOT & $U$ & 663.2 & $19.67 \pm 0.10$ \\
2009 Sep 27.91 & 1.7349 & UVOT & $U$ & 735.0 & $19.74 \pm 0.09$ \\
2009 Sep 27.95 & 1.7846 & UVOT & $V$ & 2168.5 & $19.82 \pm 0.09$ \\
2009 Sep 27.97 & 1.8018 & UVOT & $U$ & 737.0 & $19.71 \pm 0.09$ \\
2009 Sep 28.04 & 1.8685 & UVOT & $U$ & 742.9 & $19.78 \pm 0.10$ \\
2009 Sep 28.11 & 1.9344 & UVOT & $U$ & 577.3 & $19.79 \pm 0.11$ \\
2009 Sep 28.12 & 1.9476 & UVOT & $U$ & 341.3 & $19.73 \pm 0.14$ \\
2009 Sep 28.40 & 2.2343 & UVOT & $U$ & 1329.2 & $20.13 \pm 0.08$ \\
2009 Sep 28.55 & 2.3829 & UVOT & $U$ & 1730.2 & $20.01 \pm 0.07$ \\
2009 Sep 28.56 & 2.3950 & UVOT & $V$ & 1131.6 & $20.07 \pm 0.14$ \\
2009 Sep 28.88 & 2.7199 & UVOT & $U$ & 2642.7 & $20.11 \pm 0.06$ \\
2009 Sep 28.89 & 2.7277 & UVOT & $V$ & 2417.0 & $20.11 \pm 0.10$ \\
2009 Sep 29.08 & 2.9301 & PROMPT-5 & $I$ & 3200.0 & $19.48 \pm 0.10$   \\
2009 Sep 29.08 & 2.9346 & PROMPT-4 & $R$ & 2560.0 & $19.96 \pm 0.12$   \\
2009 Sep 29.13 & 2.9642 & PROMPT-5 & $I$ & 1840.0 & $19.39 \pm 0.11$   \\
2009 Sep 29.13 & 2.9644 & PROMPT-4 & $R$ & 1840.0 & $19.88 \pm 0.12$   \\
2009 Sep 29.16 & 2.9892 & SMARTS / ANDICAM & $I$ & 2160.0 & $19.53 \pm 0.07$ \\
2009 Sep 29.16 & 2.9892 & SMARTS / ANDICAM & $J$ & 1800.0 & $18.35 \pm 0.09$ \\
2009 Sep 29.17 & 3.0041 & PROMPT-5 & $I$ & 2720.0 & $19.47 \pm 0.10$   \\
2009 Sep 29.17 & 3.0055 & PROMPT-3 & $B$ & 3520.0 & $> 21.85$   \\
2009 Sep 29.17 & 3.0056 & PROMPT-4 & $R$ & 2960.0 & $19.85 \pm 0.09$   \\
2009 Sep 29.17 & 3.0083 & PROMPT-2 & $V$ & 3600.0 & $> 20.94$   \\
2009 Sep 29.53 & 3.3664 & UVOT & $V$ & 2533.9 & $20.75 \pm 0.13$ \\
2009 Sep 29.54 & 3.3796 & UVOT & $U$ & 3233.8 & $20.58 \pm 0.07$ \\
2009 Sep 30.00 & 3.8439 & PROMPT-5 & $I$ & 5840.0 & $19.78 \pm 0.11$   \\
2009 Sep 30.00 & 3.8446 & PROMPT-4 & $R$ & 6560.0 & $20.28 \pm 0.10$   \\
2009 Sep 30.08 & 3.9295 & PROMPT-5 & $I$ & 6000.0 & $19.84 \pm 0.12$   \\
2009 Sep 30.08 & 3.9302 & PROMPT-4 & $R$ & 5680.0 & $20.54 \pm 0.14$   \\
2009 Sep 30.17 & 4.0116 & PROMPT-3 & $B$ & 30640.0 & $21.74 \pm 0.13$   \\
2009 Sep 30.17 & 4.0121 & PROMPT-2 & $V$ & 28720.0 & $20.98 \pm 0.17$   \\
2009 Sep 30.17 & 4.0249 & PROMPT-5 & $I$ & 7440.0 & $19.99 \pm 0.12$   \\
2009 Sep 30.17 & 4.0253 & PROMPT-4 & $R$ & 7520.0 & $20.44 \pm 0.09$   \\
2009 Sep 30.29 & 4.1428 & PROMPT-5 & $I$ & 10400.0 & $20.07 \pm 0.11$   \\
2009 Sep 30.29 & 4.1445 & PROMPT-4 & $R$ & 10400.0 & $20.62 \pm 0.10$   \\
2009 Sep 30.55 & 4.3878 & UVOT & $V$ & 3091.7 & $20.60 \pm 0.11$ \\
2009 Sep 30.55 & 4.3944 & UVOT & $U$ & 3341.7 & $20.90 \pm 0.08$ \\
2009 Oct 1.04 & 4.8842 & PROMPT-4 & $R$ & 12640.0 & $20.62 \pm 0.10$   \\
2009 Oct 1.04 & 4.8854 & PROMPT-5 & $I$ & 12400.0 & $20.06 \pm 0.10$   \\
2009 Oct 1.11 & 4.9658 & SMARTS / ANDICAM & $I$ & 2160.0 & $20.33 \pm 0.10$ \\
2009 Oct 1.11 & 4.9658 & SMARTS / ANDICAM & $J$ & 1800.0 & $19.16 \pm 0.13$ \\
2009 Oct 1.13 & 4.9841 & PROMPT-2 & $V$ & 23520.0 & $> 21.84$   \\
2009 Oct 1.17 & 4.9896 & PROMPT-3 & $B$ & 24240.0 & $21.77 \pm 0.17$   \\
2009 Oct 1.25 & 5.1003 & PROMPT-5 & $I$ & 12640.0 & $20.06 \pm 0.11$  \\
2009 Oct 1.25 & 5.1024 & PROMPT-4 & $R$ & 11920.0 & $20.81 \pm 0.13$   \\
2009 Oct 1.64 & 5.4915 & UVOT & $U$ & 4142.8 & $21.36 \pm 0.10$ \\
2009 Oct 2.04 & 5.8878 & PROMPT-4 & $R$ & 11600.0 & $20.72 \pm 0.11$   \\
2009 Oct 2.17 & 5.9904 & PROMPT-2 & $V$ & 21360.0 & $> 21.74$   \\
2009 Oct 2.17 & 6.0045 & PROMPT-3 & $B$ & 28400.0 & $> 22.75$   \\
2009 Oct 2.25 & 6.0812 & PROMPT-4 & $R$ & 16960.0 & $20.93 \pm 0.11$   \\
2009 Oct 2.25 & 6.0880 & PROMPT-5 & $I$ & 15040.0 & $20.50 \pm 0.15$   \\
2009 Oct 3.00 & 6.8605 & PROMPT-4 & $R$ & 4240.0 & $> 21.23$   \\
2009 Oct 3.04 & 6.8617 & PROMPT-5 & $I$ & 4000.0 & $> 20.54$   \\
2009 Oct 3.04 & 6.8650 & PROMPT-3 & $B$ & 3520.0 & $> 21.45$   \\
2009 Oct 3.00 & 6.8781 & UVOT & $U$ & 8789.3 & $21.59 \pm 0.08$ \\
2009 Oct 4.13 & 7.9690 & PROMPT-5 & $I$ & 320.0 & $> 17.84$   \\
2009 Oct 4.13 & 7.9692 & PROMPT-4 & $R$ & 320.0 & $> 18.53$   \\
2009 Oct 4.13 & 7.9692 & PROMPT-3 & $B$ & 320.0 & $> 19.05$   \\
2009 Sep 4.74 & 8.5887 & UVOT & $U$ & 4052.7 & $22.09 \pm 0.18$ \\
2009 Oct 5.17 & 8.9975 & PROMPT-4 & $R$ & 12400.0 & $> 21.73$   \\
2009 Oct 5.17 & 9.0014 & PROMPT-5 & $I$ & 13280.0 & $> 21.24$   \\
2009 Oct 5.49 & 9.3449 & UVOT & $U$ & 4640.7 & $22.07 \pm 0.16$ \\
2009 Oct 6.38 & 10.2257 & UVOT & $U$ & 4392.5 & $22.84 \pm 0.29$ \\
2009 Oct 7.17 & 11.0096 & PROMPT-4 & $R$ & 27840.0 & $21.98 \pm 0.22$   \\
2009 Oct 7.21 & 11.0377 & PROMPT-5 & $I$ & 23680.0 & $> 22.04$   \\
2009 Oct 7.42 & 11.2777 & UVOT & $U$ & 5096.2 & $22.22 \pm 0.17$ \\
2009 Oct 8.32 & 12.1742 & UVOT & $U$ & 4573.2 & $22.94 \pm 0.33$ \\
2009 Oct 19.05 & 22.90 & Gemini-S / GMOS & $g^{\prime}$ & 600.0 & $24.56 \pm 0.11$ \\
2009 Oct 19.05 & 22.90 & Gemini-S / GMOS & $r^{\prime}$ & 600.0 & $23.97 \pm 0.11$ \\
2009 Oct 19.05 & 22.90 & Gemini-S / GMOS & $i^{\prime}$ & 600.0 & $23.67 \pm 0.12$ \\
%
\enddata
\tablenotetext{a}{UT at beginning of exposure.}
\tablenotetext{b}{Time from midpoint of exposure to \fermi-GBM trigger.}
\tablenotetext{c}{Reported magnitudes have not been corrected for Galactic extinction
   ($E(B-V) = 0.024$\,mag; \citealt{sfd98}).  Observations in the $g^{\prime}$-, $r^{\prime}$-,
   and $i^{\prime}$-bands are reported on the AB magnitude system \citep{og83}.  All other
   filters are referenced to Vega.}
\label{tab:0926aopt}
\end{deluxetable}

